Designing a User-centric Framework for Information Quality Ranking of Large-scale Street View Images

Street view imagery (SVI), largely captured via outfitted fleets or mounted dashcams in consumer vehicles is a rapidly growing source of geospatial data used in urban sensing and development. These datasets are often collected opportunistically, are massive in size, and vary in quality which limits the scope and extent of their use in urban planning. Thus far there has not been much work to identify the obstacles experienced and tools needed by the users of such datasets. This severely limits the opportunities of using emerging street view images in supporting novel research questions that can improve the quality of urban life. This work includes a formative interview study with 5 expert users of large-scale street view datasets from academia, urban planning, and related professions which identifies novel use cases, challenges, and opportunities to increase the utility of these datasets. Based on the user findings, we present a framework to evaluate the quality of information for street images across three attributes (spatial, temporal, and content) that stakeholders can utilize for estimating the value of a dataset, and to improve it over time for their respective use case. We then present a case study using novel street view images where we evaluate our framework and present practical use cases for users. We discuss the implications for designing future systems to support the collection and use of street view data to assist in sensing and planning the urban environment.

==> discussions_old.tex <==
\section{Discussion}

\subsection{Cost and Availability} \label{sec:discussion_cost}
The period of free access to GSV demonstrated applications and use cases that GSV's current cost structure no longer supports. There are therefore opportunities for parties who can provide open-source or low-cost datasets to fulfill urban planning, analysis, and research needs.  P5 mentioned how the change in Google street view pricing affected their research.
As several participants mentioned, high costs for evaluating the quality and potential value of street view data present barriers to the use of SVI by urban planning professionals.   

The list of existing high-frequency street view data providers includes permissively licensed images collected by crowd-workers, and proprietary data collected by sensors installed by OEMs and aftermarket vehicle products. The growth of public datasets could parallel the arc of freely available high-frequency remote observation data from sources such as Landsat, and the Copernicus Program. These datasets have resulted in numerous publications in urban studies and planning \cite{cetin2019effect, deliry2021extracting, fu2019characterizing, jutz2020copernicus, tapete2018appraisal, kuc2019sentinel} as well as other fields. The value of this data likely led to much of the growth of the private and commercial remote observation industry \cite{dehqanzada2000secrets, wulder2019current}. 
% ranging from agriculture \cite{}, OSINT \cite{}, finance and international relations

\subsection{Tooling and Interfaces}
% continue in the challenges discussed when it comes to tools and interfaces for high frequency street view imagery. Both are massive image datasets that can be difficult to work with.
Interacting with large imagery datasets of all kinds remains challenging. While there have been some approaches as discussed in section \ref{sec:background_human_centered}, images can be noisy, and require large amounts of storage and processing power for analysis. While deep learning techniques for image analysis, segmentation, and object recognition have improved significantly since the 2010's \cite{alom2018history}, many challenges remain when problem areas aren't tightly bounded, which is often the case in urban analysis.
Some of the parallels to satellite imagery observations in section \ref{sec:discussion_cost} are also productive for developing the space of tools and interfaces for street view datasets. Similar to the field of remote observation, the data is imagery in massive quantities. The mode of analysis is often exploratory and may require expert labeling. Both satellite and street view imagery raise persistent privacy concerns that individuals, states, and corporations will be forced to navigate. Some of the tooling that has been developed by the remote observation community points towards similar approaches that might scale to the challenges of street view imagery.

Platforms and infrastructure such as Google Earth Engine \cite{gorelick2017google} and Sentinel Hub \cite{milcinski2017sentinel} demonstrate how massive parallel computing can be made easy and accessible to novices democratizing analysis. They also include pricing structures that make non-commercial, academic and government use affordable or free further incentivizing their use.

More accessible and collaborative software for generating custom maps \cite{kastanakis2016mapbox, felt, placemark} is beginning  to address some of the requirements of community organizations as described by P2 and P3. Some data providers are beginning to integrate tooling for custom maps, filtering by object detection, and easier data exploration. While these tools are still limited, %object detections are only available from predetermined categories. S
some of the exact problems and uses described by P3 and P5, such as curbside detection, are already beginning to be offered by companies such as Nexar \cite{nexar_2021}. We can expect these tools to continue to improve and add functionality.
\begin{figure}[t]
     \centering
     \begin{subfigure}[b]{0.48\textwidth}
         \centering
         \includegraphics[width=\textwidth]{Figures/mapillary_filters.png}
         \caption{Mapillary filtering for cars, bicycles, and cyclists \cite{mapillary_2019}}
         \label{fig:mapillary_od}
     \end{subfigure}
     \hfill
     \begin{subfigure}[b]{0.46\textwidth}
         \centering
         \includegraphics[width=\textwidth]{Figures/nexar_filters.png}
         \caption{Nexar CityStream filtering for traffic signs \cite{nexar_2022}}
         \label{fig:nexar_citystream}
     \end{subfigure}
     \caption{Filtering for detected objects in street view images.}
\end{figure}

\subsection{Value and Quality of Street View Imagery} 

Images contain `general-purpose' information with many use cases. However, the quality of crowd-sourced images varies due to heterogeneity in device, orientation, and occlusions. Data collected in uncontrolled settings can show spatial, temporal, and content distribution variance. Images may be of sufficient quality for some applications while needing a higher quality score for others. Collecting more information or maximizing coverage does not guarantee improved data quality. For example, air quality changes slowly, so a higher sampling frequency may not add more value to the data in regular environmental sensing applications. Evaluating the value and relevancy of data is essential to justify the monetary and labor investment urban professionals need to sanction before incorporating such large-scale datasets into their analysis workflow.

Quality of Information in a sensor network is a metric used to evaluate information to make decisions about the utility of a specific piece of information \cite{10.1145/2489253.2489265}. It is the difference between observed measurements of an event via sensing and the actual measurement \cite{4660116, 10.1016/j.cageo.2021.104991}.
Frameworks have been proposed for scoring and ranking generic information based on spatio-temporal context, accessibility, trustworthiness, data provenance, timeliness, presentation, and relevance as key characteristics to evaluate application-specific utility \cite{10.1145/2489253.2489265}. Existing approaches have developed application-specific frameworks by ranking sensors according to task relevancy and user requirements  \cite{8606228, 6935003, 7295461, 7348644}. 
The quality of coverage thus depends on the velocity, mobility pattern, and the number of sensors available \cite{10.1145/1161089.1161102}. Existing work has explored adaptive spatial sampling for optimizing value and cost \cite{BALLARI2012102, NGAI2014203}, and detecting missing points in data to improve coverage \cite{wang2006movement}. 

Most existing works focus on spatial coverage, and little work on Quality of Information has focused on temporal coverage, where events of interest need to be observed multiple times within a time interval.  
The large volume of data generated by such vehicular networks is a challenge due to the processing and storage requirements. These may be mitigated by querying and filtering data points below certain information quality (e.g. filtering images in dark, occlusion, blurriness, etc. conditions). Data-driven mechanisms need to be formulated to localize data segments with low information quality and incentive mechanisms produced to improve the quality of captured imagery~\cite{10.1145/2888398}.



% hile some services such as GSV ensure spatial coverage updated approximately least once per year, data collected at this frequency can  be less relevant to detect changes in urban aspects that change at a faster temporal rate. On the other hand, w

% When multiple instances of the same event are captured, the Quality of Information for each capture must be determined to decide which instance is prioritized. This is particularly challenging when sensor samples are images, whose content may be of high quality and relevancy for one context while providing low information value for another (e.g. image of the same road intersection showing the potholes of the street may be less valuable for pedestrian counting applications). 

% It is closely related to Value of Information \cite{article12}, a concept to assess the utility of information for a specific purpose.
% , and Age of Information \cite{yates2021age} which is the concept of timeliness of information delivery. 
% Quality of information can be regarded as context-independent whereas the value of information is context-dependent. Even high information quality can offer low information value for a specific application \cite{4144841, bisdikian2007quality} 
% (e.g. temperature data at minute resolution for transit design).  
% As the definition of information value is dependent on the specific purpose where it is used, evaluating the Quality of Information across multiple applications is challenging. 


% Quality of Information is influenced by external environmental factors, 


% The quality of information from mobile sensing systems that capture, street view images is dependent on the dynamism inherent in the network.


% As spatiotemporal data collected by vehicular networks, street view image data can be considered a form of participatory sensing \cite{burke2006participatory, 10.1145/2888398}. As humans and external factors such as social, economic, and cultural context are major actors in the data collection, trustworthiness, reliability, and consistency needed for adequate information quality is crucial as outlined in \cite{10.1145/3139256}. 


% Although there are various Quality of Information measures proposed in the literature that can be useful for sensing data at a city scale, there is little work to measure information quality for Spatio-temporal data. It is particularly challenging when the data is collected in image form as information quality that can be extracted from an image is application specific. It is becoming increasingly popular to use computer vision to automatically extract information from large-scale street datasets to develop insights for planning and policies. Without a proper mechanism to evaluate the quality and value of the data for the task in hand, the data can provide an incomplete understanding of the city and its population leading to unfair policies and planning decisions.



\subsection{Privacy and Equity}
Privacy concerns with on-street image collection have a long precedent as discussed in section \ref{sec:background_privacy}. Most publicly licensed street view imagery (Mapillary and KartaView) have followed Google's precedent, blurring faces and identifiable information. While P2 considered the removal of all people from images to mitigate privacy concerns as discussed in section \ref{sec:findings_privacy}, many of their suggested use cases would conflict with that. For example, SVI datasets can have such high spatial density and image frequency that a person could be tracked via their clothing even if their face is blurred. Further work is necessary to understand the potential privacy harms that high frequency street view data might pose. Existing approaches to mitigate privacy harms--such as similar pedestrian substitution \cite{nodari2012digital} or image-to-image translation \cite{xiong2019privacy}--may also be applicable to these datasets. Furthermore, we should acknowledge there are sensitive sites-- parenthood clinics, dispensaries, bars, playgrounds-- that present risk to different populations around which active regulation of data collection may be necessary.

One of the benefits of imagery at this scale and temporal frequency is the ability to capture data on demand when you need it for a specific research goal rather than storing everything. On the other hand, for things like understanding historical trends or response to specific events--like how people respond to a public health curfew in different neighborhoods--having caches of data going back to specific times can be very useful. In some ways, having collections of "normal" behavior, lightly sampled, and adding temporal resolution and density of coverage when patterns are unusual is what might be most useful for detecting urban patterns and responding proactively to new issues or patterns. 

Ensuring fresh and equitable imagery will require broad infrastructural investment or  a well-formulated incentive structure for crowd-contributed data. Mapillary has a marketplace and ``Missions'' to fund and gamify data capture \cite{quack_2021}. Both KartaView and Mapillary publicly display leaderboards to encourage participation and data collection. These incentive structures may help but are insufficient with Mapillary still showing significant inequality in data captured \cite{ma2019state}. Collaborations with fleets and state agencies that already have consistent and full coverage may help guarantee more equitable coverage \cite{yoong_2018}.


\subsection{Limitations}

Our interviews are based on a single SVI dataset as an example. The images in the dataset is primarily collected in North America. The interviewed professionals all are based in New York, USA. The reader may concern that we have five participants taking part in the interview study. However, based on our thematic analysis we found five participants to be sufficient to reach convergence. 
% Notes from chat
% this is stuff that you can just collect on demand (privacy). GSV is secondary use, it can be useful or abusive. If you can get a lot of data on demand you can capture the data on demand when you need it. On the other hand, for things like understanding historical trends or response for specific events--like how people respond to a public health curfew in different neighborhoods--having caches of data going back to specific times can be very useful. In some ways, having collections of "normal" behavior, lightly sampled, and adding temporal resolution and density of coverage when patterns are unusual is what might be most useful for detecting urban patterns and responding proactively to new issues or patterns. 

%Otherwise, having filters on for commonly abusable information which enables individual level tracking and having some log of people who ask to pull requests for that data to be off might be helpful for having people think twice about hoarding potentially abusable information, and at least encouraging accountability and transparency about how the data is used.


% I think it’s worth saying that it is possible to have loss of privacy, but that the likelihood of catching any specific person using these methods is low, since the capture of individuals with these methods is serendipitous.
% Nevertheless there are sensitive sites—parenthood clinics, dispensaries, bars, playgrounds—that we should be mindful might present risk to different populations, and hence some proactive anticipation and mediation of possible issues is necessary




==> findings_old.tex <==
%reframe with novel use cases that is currently unsupported
\section{Findings from Expert Perspectives}


We identify a number of themes  related to the differences between participant approaches to novel datasets, previous experience with street view imagery, and the application areas they explore around the potential uses of dash cam street view imagery. Participants regularly framed the challenges and opportunities relative to their experience with existing datasets such as GSV. While several of the challenges noted are not unique to street view imagery, these challenges are often exacerbated by the data-set sizes and the quality variance presented by dash-cam footage. We present the findings below.

\subsection{Financial Cost} \label{sec:findings_cost}
Deciding to use a data product is intimately related to its cost. Cost of access and cost of use can be prohibitive to organizations, particularly when researchers are uncertain if they will be able to extract relevant outputs.

% \subsubsection{ Costs}

P2 described the selection and procurement process at the New York Department of City Planning:
\textit{\begin{quote}
    There were a few times where [we used] proprietary data sets. However, they were either just too expensive for a city budget and you have to go through a whole procurement process that can open up a can of worms... Trying to assess, how much value we would really get for this proprietary data? Is it really worth that cost? Whether it's a financial cost or the labor costs of doing this procurement process.
\end{quote}}

Government resources are limited and data procurement involved enough work that it was often better to ``scale back [P2's] expectations or scope of our work and still kind of generally get to the right direction, of the kind of analysis we're trying to do with just open data sets.'' Data for governmental, non-profit, or community organizations would better serve the public if the data is permissively licensed or easily accessible to researchers and urban planners who might work in these areas.

The issue of cost was echoed in P5's description of changes in GSV data from free data to a limited and priced credit system:
\textit{\begin{quote}
    Google started to charge for images. That made a huge difference for academics who want to use it...  Now I think  [GSV] account only gives users  200 credits per month.
\end{quote}}

The restrictions on data usage affected the degree to which academics could rely on GSV and motivated a turn to other sources. When operating with access to large resources in a collaboration on a well-funded project, P5 described the affiliates that enable bulk downloads of GSV data:
\textit{\begin{quote}
    [They] were rich enough to say `I want all the data'...  it's a company that works closely with Google, for people to get a large quantity of the data. The first million images is expensive, but additional millions of images is much cheaper. [This] gives researchers less motivation to query the data.
\end{quote}}

The pricing structure described above is designed to encourage bulk downloading. The result is to privilege institutions with pre-existing relationships with large corporations, large onsite or cloud storage facilities, access to a supercomputer, and a predetermined question rather than exploratory analysis.

P4 noted how costing processes change as a dataset becomes more useful:
\textit{\begin{quote}
     The value of a data set changes based on the competition. There's also a barrier, where, if [the data] gets too expensive, people are just going to not care anymore, and find another way to do it. Or start collecting data [themselves]. ... If it's free and low-hanging fruit, it's really exciting because there seems like there is big potential. Once that paywall gets introduced ... it seems to be less useful. It seems to just fall into the business bottle of some company and then it's a black hole.
\end{quote}}

Proprietary datasets are already being used in the service of generating a profit while permissively licensed datasets are currently owned by large corporations with no guarantees those datasets will remain openly accessible. 

% \subsubsection{Computational Costs}
% \subsubsection{Labor Costs}
% Choices on data sources and types to use are 
% \subsection{Expertise and Infrastructure}  \label{sec:findings_infrastructure}

\subsection{Static vs Dynamic Spatial Attributes}  \label{sec:dynamic}

Participants focused on application areas that were suited to lower quality images with much higher update frequencies. These were often brought up in direct contrast to GSV. Google cars typically revisit a street around once or twice a year, often optimizing for times when the street is the least busy. This limits the ability to use their data for understanding aspects of the urban environment that change faster than that or focusing on people and objects moving through the space rather than aspects that are fixed and infrastructural.

P3 described sending staff weekly to survey charges to retail spaces on the ground level, currently taking up to 20 person-hours of labor a week using ``a spreadsheet they actually print out and walk around with and check on things''. While P3 had recently used street view to check ``if there were manhole covers on the street'' which were covered in snow at the time, P3 stated that their staff would ``never lean on it for on-the-ground measurements or anything.'' GSV is a tool primarily for when they are ``being lazy'' or viewing something far from the district. However, P3 and their organization find value in real-time data sources when insights were extracted for them. Using a service called Spring-Board, three cameras installed at high angles in parks are used for pedestrian counts \cite{springboard_2022}. Given the use of existing statically mounted cameras, there is a clear use case for pedestrian tracking and understanding foot traffic behavior in this Business Improvement District.

The eye-level perspective of SVI allows for a better understanding and analysis of fine-grained human behavior in space than street view datasets captured from high angles. P2 described: % how part of the job of an urban designer included:
\textit{\begin{quote}
   [Part of the job of an urban designer is understanding] how do people move through the space. Do you notice that a lot of people sit there? Are there always constantly groups of people sitting around? Or is there always a steady flow of people walking through the space? I would also [pay attention to] cyclists. Are there any cyclists moving through space? Are they locking their bikes anywhere?
\end{quote}}

As discussed in Section \ref{sec:background}, fine-grained canvasing is historically labor-intensive, and demands an observer to be on-site  for extended periods of time. Higher frequency capture of street view imagery may open up new methods for urban analysis at scale.

P3 described several observations that would have been easier to deduce via street view imagery rather than manual counts.
\textit{\begin{quote}
    While [looking at] quantity counts of bike traffic in the district during the summer, I expected that people would be biking in the morning and evening. In reality, it was actually lunchtime and evening. What I realized pretty quickly was the bike traffic was largely commercial cyclists at lunchtime, making deliveries. We also saw that Broadway was about 25\% bidirectional biking even though it's a one-way facility. People are using it both ways because it's so convenient as a diagonal.
\end{quote}}

Urban environments are used in ways that were not originally intended. Better instrumentation of the urban landscape allows the urban design to adapt to the norms people develop as they move about space. P3 continued to describe how they hoped to add additional bike parking in response to the massive influx of food delivery workers. Being able to capture and query this kind of data on demand would aid that process.

Participants described other counter-intuitive temporal data that they believed could be extracted from street view imagery. Describing the need for increased granularity to assist older adults, P1 mentioned this:
\textit{\begin{quote}
     [Beyond bi-weekly updates], it could be even more granular. Even time of the day. If [an elderly person] live[s] across the street from a school, most of the time walking in that community is not a problem. But when the kids are leaving school at three o'clock or right before school starts there's no way that [they] can get access. It could even be more granular a whole day, it could be times of the day... [also] seasonality. This block could be fine nine months out of the year, but three months out of the year, it's treacherous.
\end{quote}}
 
 Temporal granularity can raise causal relationships that might otherwise be challenging to deduce. Seeing exemplar data that is updated in near real-time led P1 to suggest building new kinds of tooling that could assist elderly inhabitants to decide when to leave or how to navigate the city that takes their unique needs into account.
 
 Higher update imagery can also benefit urban populations more generally. P5 noted how urban developments such as ride-sharing and e-scooters have complicated how cities prioritize curb use:
\textit{ \begin{quote}
     [Another field] that is developing very rapidly is curbside parking, or curb use. It has become a very popular problem, especially after the introduction of micro-mobilities [scooters and e-bikes], and Uber. You frequently see Uber drivers double-park, loading and unloading. A lot of places are trying to get rid of on-street parking which frees up the curb spaces [reserved for] loading and unloading only. It's a very vague criteria. How do you define how long people park there? What would be considered as loading and unloading? Is sitting there for 30 minutes loading or unloading? That's very hard to decide...[these kinds of] reinforcement things would benefit from images that update more frequently
 \end{quote}}
 
%  So all those kind of reinforcement thing would benefit from the image that is updating and also like the real-time traffic information that will be extracted and all the congestion, emission data that can be. provided on those kind of image will be also very valuable... there are projects that try to predict air quality based on Google Street View image. Then if it's updated every second, every minute, it will have better air quality model.

Of the many use cases for street view imagery discussed in section \ref{sec:background}, many of them would benefit from higher frequency data if the underlying signal extracted changes at a time frame greater than the once every 6-12 months GSV and related projects typically re-image a street. P5 added that ``projects that try to predict air quality based on Google Street View images, if it's updated every minute, will result in a better air quality model.''

Similar to the examples mentioned in section \ref{sec:background_urban_computing}, changes in street assets due to damage were raised by P4, P3, and P5. P3 and P5 mentioned that many municipalities have no consistent database of traffic signs. If one is knocked over in the Flatiron District, P3 or someone from their team reaches out to the Department of Transportation to get it fixed. It is worth noyting that some of these opportunities are afforded today using street view imagery, such as to better keep track of road and traffic signs, and curb usage~\cite{nexar_2022}.

\subsection{Interacting with images at scale} \label{sec:findings_image_scale}
Large amounts of image data provide unique challenges to both the quantitative and qualitative analytical methodologies used by our participants. This includes data exploration, storage, labeling, filtering, querying and reporting. 

P2 further describes the importance of street view imagery and the failure in tooling to bring together imagery and analysis that urban planners can use:
\textit{\begin{quote}
    The reason why a lot of photos are required for city planning or zoning applications is because you can read a lot from photos of places in the city. I just haven't seen yet a lot of tools that make that connection. [Tools that try] to further analyze the data that [urban planners] are reading from these photos. 
\end{quote}}

% I think oftentimes a lot of its inferred or it just has to be written out exactly what's what's valuable about this particular image.

Until tooling improves the opportunities for urban analysis at scale is unlikely to occur. Urban planners and analysts need methods for approaching large datasets that can be queried and clustered for use patterns. 

P2 described how making tools for community organizations required simple clear outputs that could be used with little modification:
\textit{\begin{quote}
    [Community board members] weren't data experts per se, they just have these reports. The biggest challenge that they had is that the open data portal seemed overwhelming. They're not comfortable with spreadsheets. They have these reports, but they're often outdated. The reports [may not contain] the specific types of data that they want to report. Instead of saying the top three languages spoken, they want to be able to at least have the option to provide top 15 languages spoken in their neighborhood, and that may not have been provided. That particular audience honestly just want the visualization...to maybe copy and paste specific data points that were helpful for their work. They were also able to easily create screenshots of graphs, or custom maps...that they can put in their report. That was really valuable for them.
\end{quote}}

For users less confident in interacting with large datasets `` the biggest value was really the ability to visualize data and do some slight customization of like maps and graphs'' (P2).

The process P2 described aligned with the approach taken by P3 which involved a number of tools that take complex inputs and produce direct readable reports stating ``we're still pretty dependent on the dashboards that we actually pay for and we keep those reports''. P2 mentioned Spring-board which uses mounted cameras and computer vision to generate pedestrian counts. CoStar merges a variety of public information to generate reports on real estate. Placer.ai is used to estimate foot traffic in the neighborhood. StreetPlus generates a data dashboard for waste management. These services are paid for and used to simplify data collection and analysis by a team that is small and unlikely to employ a data scientist.
 
P1 considered the utility of being able to query images which could then be used for ``validating that data with older adults and workshops where [we would like to ask participants ]`Hey can you point out some problematic areas for us?' ''. The opportunity presented allows street view imagery to be leveraged as a probe to better discuss the challenges of elderly residents, challenges which may or may not be reflected in the existing data.
% Our experts came from a range of backgrounds with various amounts of exposure to data science. 

Visual data often requires labeling to extract information not captured by simple heuristics. This is a well-explored challenge in HCI, CSCW, and AI communities which some of our participants have first-hand experience with. For simple labeling tasks, P5 is having Mechanical Turk workers draw bounding boxes around e-scooters. For more complex tasks, P5 describes:
\textit{\begin{quote}
    We have been using Mechanical Turk to label the sample data to develop machine learning models using Street View to predict Local Climate Zone... Mechanical Turk is highly scalable. We can gather those results fairly quickly, but the quality of the results is not comparable with expert labeling.
\end{quote}}

A significant amount of work is necessary to make street view datasets usable. For features without obvious heuristics, each labeling task will differ based on the application. If each feature of interest requires expert labeling, the likelihood of widespread use is limited. 

% \subsection{Ethical Concerns}  \label{sec:findings_ethics}

% The datasets being described are urban surveillance at a massive scale. Ethical concerns brought up existed primarily along two tracks. There were concerns about maintaining privacy and the potential reduced utility of the datasets that might pose. The other theme that was brought up was data equity and curation. Given that these datasets are collected from vehicles the limit is areas where there may be fewer cars. In particular Nexar has many dash-cams mounted in ride-share vehicles which many not serve all areas.

\subsection{Privacy} \label{sec:findings_privacy}

In general, participants approached the datasets as an opportunity in their own work and were less concerned with some of the significant privacy violations made possible by such massive imagery datasets.

P2 was a key exception to that pattern. While P2 had described much of the value of street view imagery as being related to how the imagery captures people interacting in public, P2 were also hesitant. P2 described how standard privacy mitigation for public imagery may be insufficient:
\textit{\begin{quote}
    Even though faces might be blurred, because this data is captured at a higher frequency, it's still easy to see patterns. For people living on [a] block, you might see them ... multiple times a day.  I do think that blurring faces isn't enough in addressing privacy. It requires the obscuring of people in general. Because again, you're able to start picking up on patterns and triangulating data.
\end{quote}}

 Given P2's background working with the government and with community groups, underrepresented minorities and people of color, they were the most concerned about the potential for privacy abuses by state, corporate and individual actors. Maintaining privacy is an important area that will require additional study if large scale street view datasets are to be made a viable resource for urban studies.

Longstanding concerns around privacy with GSV were discussed in section \ref{sec:background_privacy}. Many of these concerns may be exacerbated as the size of these datasets grow; the temptation to use these large-scale urban datasets "for good" with the belief that such uses can be separated from the bad uses still seems to prevail. 

P5, for example, seemed critical of privacy protections, and seemed to indicate that more surveillance could be used to address crime. 
\textit{\begin{quote}
    [Be]cause United States doesn't have a security surveillance system due to privacy protections, sometimes you really need, those kind of images to, know whether a crime really happened. Or if a crime happened, where that person went. If you have good coverage and videos that is updated frequently enough, you can leverage it as a security system for the city.
\end{quote}}

 To us, this is an indicator that researchers and planners who have access to large scale urban datasets might, with only good intentions, enable data usage that violates people's civil liberties if potential abuses are insufficiently managed. This type of misuse should be anticipated and addressed %The desire to use these tools for the enforcement of a carceral state will need to be taken into account 
 by those that produce, release, and sell these datasets.

\subsection{Data Equity and Curation}
% \subsubsection{Access and Resource Equity}
If data is being used to make claims, and enact policy changes, it requires guarantees about its completeness and distribution. Data needs to be collected such that it controls for temporal and spatial differences. If an area is being sampled more frequently end users should be able to easily control for that in their analysis to reduce oversampling bias. 

P4 referred to previous work that showed:
\textit{\begin{quote}
    If [researchers randomly put a sensor on 30 taxis, within 24 hours it would cover every block [in Manhattan] so just pick 30 taxis at random and that's all it would take to at least get to each block once, roughly speaking of course.
\end{quote}}

Increasing the number of sensors placed on vehicles increases both the spatial and temporal frequency of data collection. This is one approach to ensuring data is widely cross-applicable.

When working on a project, P2 described the process of curating interviews: 
\textit{\begin{quote}
    [Curating interviews require being] strategic and finding specific people who, represent broadly across different demographics. When I talked to city planners...  I tried to find people of different demographics, people of color, older people, younger people... Not only do we identify the most appropriate people for our work but we're trying to make sure we have a broad cross-section of demographics when inviting people for interviews.
\end{quote}}

P2 is suggesting that the same approach to curating interviews in more ethnographically focused work could provide an approach to the curating of street view datasets. Collect images that target the specific groups, locations, and demographics necessary to effectively answer the question rather than attempting to collect any and all data available with the expectation that it will immediately be useful.
% Curating interview subjects as a model for intentionality in dataset curation is reflected in some of P2's concerns with how data around walkability is typically defined rather than used in practice.
\textit{\begin{quote}
     [Often] the way that walkability is calculated isn't actually a helpful way to assess particular subgroups of walkers like elderly people.  I find that that circumstance is true for lots of other city residents ...I've personally experienced how limited data can be because, it's either captured in a way that's just too broad, or that it is only really relevant for an athletic young male  city dweller.
\end{quote}}

When large datasets are utilized to determine whether a metric that might be ageist, ablest or presupposes a norm, it doesn't matter how large the data originally was. P2 points out:
\
\textit{\begin{quote}
    [It is better to] not just have more data available, but to specifically toggle to specific subsets of demographics. [Finding] data that's most relevant to those subsets would be really helpful. Trying to understand what demographic subsets can you then find specific data around? and what are the limitations of that kind of data? ... Being able to capture and find data that's most relevant to very specific groups of people is helpful.
\end{quote}}

% , and can now then open up a whole floodgate of very like different ways and metrics that are most relevant to that data group that could just be like really difficult to be able to capture in a very accurate or consistent basis 

P2 suggests targeted street view data collection rather than aggregate collection. Specifying regions to intentionally address specific research or planning questions would reduce some of the costs (storage, compute, labor) and challenges of working with these datasets while allowing researchers to make equity claims directly when curating a dataset.

==> v1_CSCW/01_introduction.tex <==
\section{Introduction}
Street view image  datasets feature large numbers of images taken along streets from different locations. Unlike vertical aerial images, which might be acquired via satellite or drones, street view imagery provides scenes captured from the perspective of a human. This makes the data suitable for extracting visual features which can be of interest for estimating characteristics of the built environment such as greenery, building valuation, and pedestrian interaction in space.
Google Street View (GSV) is the best-known street view image dataset. Originally based on the Stanford City Block project, it first launched in several cities in 2007 \cite{olanoff2013inside}. In the intervening decade, GSV imagery would grow immensely, estimated to cover half of the human population by 2018 \cite{goel2018estimating}. However, there is an increasing number of alternative street view datasets, for example from KartaView, Nexar, Mapillary, and MobilEye, made possible through the growth in dashboard cameras (dashcams) \cite{madhavan2017bdd, 10.1145/3417991}. %; these are often collected from contributors using dash-cam imagery. %, and registered under permissive licenses
%With an estimated 36.1 million units sold in 2019 \cite{ariffin2021exploring}, the extreme growth in internet connected dashboard cameras (dashcams) has resulted in a corresponding growth of street view imagery data sets \cite{madhavan2017bdd, 10.1145/3417991}.
Advances in image processing techniques for tasks such as object detection, segmentation, and scene classification, along with dramatically cheaper digital storage, have increased the accessibility and utility of these large street view datasets. While researchers, and data providers are ramping up what is possible using these services, few of those researchers seem to be directly in touch with the prospective users of these tools and services in the domain of urban planning. Hence, this work seeks to aid the advancement of this promising area in a more use-inspired direction.



% move to background?
% Increasingly, street view images are being used in urban studies applications.


% As an emerging area of big data, street view images show the promise for realizing many applications from `smart cities' vision, however, there are challenges that remain in getting that vision to reality.

% Traffic images have  been used for virtual auditing, mobility tracking, and transportation applications [reference]. Street view images are a recent addition to data sources that capture scenes happening around the built environment of public streets. 

% Street view imagery has been employed to estimate demographics \cite{gebru2017using}, tree cover \cite{li2018quantifying}, real estate value \cite{glaeser2018computer} among other things.



% The reasons for the promises of Street view images (SVI) in urban studies are many-fold. First, the images provide view of a street from the perspective of a human, unlike vertical aerial images such as satellite imagery [].  This makes the data suitable for extracting visual features from the street images which can be of interest for estimating specific characteristics of the built environment such as greenery, building valuation, etc. Such measures can then be used as a proxy for modeling the quality of different life aspects including demography, housing, education, environment, economy, health, and transport. Second, the view of different locations from the perspective of a human can enable virtual built environment representation where cost effectiveness of professional auditing improves as physical field visits are replaced. Finally, as 'pictures are worth a thousand words', such large scale image collection depicting urban life help in shaping a better story to tell by an urban designer, ethnographer or a developer. The wide coverage of street view images across many countries in the world allow researchers to compare among different hotspot areas across a single city or cities from different continents, and rank them along different societal dimension for policymaking purposes.

In this work, we outline the challenges and opportunities of these large-scale street view datasets, particularly for urban planning and analysis applications. First, we pull together literature from the fields of image-based machine learning, urban planning, human-centered computing, and data science to show growing interdisciplinary awareness and usage of large-scale street view data. Then, drawing on a series of interviews with academics, urban planners, demographers, and community organizations, we explore the potential harms and benefits of crowd-sourced dash cam imagery at scale. We use the literature and first-hand expert accounts to outline how street view images can be used by government, non-profit, and community organizations to complement their data and analysis practices. Based on the themes that emerge from the interviews and literature, we then describe potential future challenges and opportunities for such data sources, using a dataset of such images collected in New York City as an exemplar. We close with research opportunities afforded by such datasets going forward and discuss ways to improve the collection and quality of data that can open up more novel research opportunities while being mindful of privacy and surveillance concerns.





% However, as with any big data comes challenges, and Street view images are no exception to it. As the physical world undergoes many changes, SVI images need to be updated regularly. At present, each Google street view image is ~50MB [], leading up to terrabytes of data storage needed over time. Such volume requires large amount of memory and storage requirement for such database, and enormous processing power for extracting information, identify patterns and visualize to understand it. For applications that require real-time analysis, data need to be updated fast enough to support analysis, and the quality of the data need to add value to the analysis. Evaluating the value is complex for such case as it involves organizing the images and relevant contextual information in a structured manner for easy, efficient visualization. This often means data needs to be filtered or sampled so that size of the data is compressed in a way that retains only information that are relevant to the task in hand. Finally, a policymaker needs to interpret the results to gather evidence from the analysis to support their decision which depends on the trustworthiness of the data. There is a growing need for delineating the variety of dimensions that influence how street view images are collected, used, analyzed, and presented  for different applications that serve various stakeholders. Likewise, Issues such as coverage, quality, and privacy can be diminishing factors in enabling services and policies that rely on SVI. The concerns over such issues can vary widely based on organizational goals and application context. 

==> v1_CSCW/02_background.tex <==
\section{Street view Image Projects and Services} \label{sec:background}

% Street view imagery relevant due to the recent growth in the datasets and sources for street view imagery. 
In this section, we review major street view imagery projects and how they differ from one another so that the range of what might be used for urban planning and analysis is made clearer. %,  how such street view imagery is used, the state of the art for large scale public space datasets collection, as well as related research in urban computing, urban studies and privacy and data governance.

% \subsection{Street view projects}
% While aerial images have long been used by urban planners to understand aspects of the city which are not captured by maps or plans--how greenery changes over time, how buildings are being modified or decaying, how streets are affected by weather--SVI provide view of a street from the perspective of a human.  This makes the data better suitable for %extracting visual features from the street images which can  such large scale image collection 
% depicting urban life; street view imagery can capture signs or activity in ways that are easily interpretable by everyday people, as well as by urban designers, ethnographers or developers. 

\begin{table}[H]
\begin{tabular}{@{}llll@{}}
\toprule
\begin{tabular}[t]{@{}l@{}}Company \\ \end{tabular}   & \begin{tabular}[t]{@{}l@{}}Founded  \\ \end{tabular} & \begin{tabular}[t]{@{}l@{}}Business Sector  \\ \end{tabular}  & \begin{tabular}[t]{@{}l@{}}Reported Dataset Size \\ Data License\end{tabular}\\ \midrule

\rowcolor{LightCyan}
\begin{tabular}[t]{@{}l@{}}KartaView\\ ~ \end{tabular}  & \begin{tabular}[t]{@{}l@{}}2009 \\ \end{tabular}         & \begin{tabular}[t]{@{}l@{}}Open Platform (Owned by Grab Holdings) \\ \end{tabular}  & \begin{tabular}[t]{@{}l@{}}384 million over 8 million km (2021) \\ CC BY-SA 4.0  \end{tabular} \\
\begin{tabular}[t]{@{}l@{}}Mapillary\\ \end{tabular}  & \begin{tabular}[t]{@{}l@{}}2013  \\ \end{tabular}        & \begin{tabular}[t]{@{}l@{}}Open Platform (Owned by Meta Platforms)\\ \end{tabular}  & \begin{tabular}[t]{@{}l@{}}1.5 billion images over 10 million km (2021) \\ CC BY-SA 4.0\end{tabular}     \\

\rowcolor{LightCyan}
\begin{tabular}[t]{@{}l@{}}Nexar  \\ \end{tabular}    & \begin{tabular}[t]{@{}l@{}}2015  \\ \end{tabular}        & \begin{tabular}[t]{@{}l@{}}Automotive safety \& Smart dash cams  \\ \end{tabular}   & \begin{tabular}[t]{@{}l@{}}4 terabytes of images (2022)\\ Proprietary\end{tabular}        \\
\begin{tabular}[t]{@{}l@{}}Mobileye \\ \end{tabular}  & \begin{tabular}[t]{@{}l@{}}1999  \\ \end{tabular}        & \begin{tabular}[t]{@{}l@{}}Advanced Driver Assistance Systems\\ \end{tabular}       & \begin{tabular}[t]{@{}l@{}}200 petabytes of driving footage (2022)\\ Proprietary\end{tabular} \\

\rowcolor{LightCyan}\begin{tabular}[t]{@{}l@{}}Google\\ \end{tabular}   & \begin{tabular}[t]{@{}l@{}}1998  \\ \end{tabular}        & \begin{tabular}[t]{@{}l@{}}Search and Ads \\ \end{tabular}      & \begin{tabular}[t]{@{}l@{}}10 million miles (2019)\\ Proprietary\end{tabular} \\ 
%\bottomrule
\end{tabular}
\caption{\label{tab:sv_projects}Notable Street View Projects}
\end{table}

% help in shaping a better story to tell by an urban designer, ethnographer or a developer. be of interest for estimating specific characteristics of the built environment. Additionally, a 'picture is worth a thousand words', such large scale image collection depicting urban life help in shaping a better story to tell by an urban designer, ethnographer or a developer. The wide coverage of street view images across many countries in the world allow researchers to compare among different hot-spot areas across a single city or cities from different continents, and rank them along different societal dimension for policy-making purposes.
\subsection{GSV and similar services}
%  A meta-analysis of street view imagery papers showed that two-thirds of academic papers used GSV image data as their source \cite{biljecki2021street}. 
The GSV API is the most common source for street view image collection. It has been used in more than 65\% of the research publications that use street view imagery in the past 20 years \cite{BILJECKI2021104217}. A majority of the images provide a 360-degree panoramic view. The service is currently active in more than 90 countries with recent expansion to some indoor spaces. The GSV API provides access to images to its users with a pay-as-you-go model. 

The easy access, omnidirectionality, and global coverage are the major factors for GSV's popularity. GSV images have been used for urban auditing \cite{10.1145/3403931}, urban privacy computing \cite{10.1145/3461702.3462525}, building recognition \cite{10.1145/2987386.2987393}, urban accessibility \cite{10.1145/3234695.3240999}, and traffic monitoring \cite{10.1145/3180496.3180638}. 

There are also several other local instances of street view image services such as Tencent (China), Microsoft Bing Maps, Cyclomedia (Europe), Yandex (Russia), etc. which provide access to street view images accessible to specific corresponding countries.  Over 80\% of papers are based on GSV combined with Baidu Total View and Tencent Street View, products which are Chinese equivalents to GSV. 

% \subsubsection{Street View Images} While aerial images can provide useful information about overall urban infrastructure through a perspective from above, seeing the city landscape from a ground level perspective analogous to human vision provide more fine-grained information. From images captured at street level, urban developers can use these micro level information from an urban scene, classify them into different components of built environment, and statistically evaluate different parts of the city for policy making purpose. As mentioned above, GSV API is the most common source for street view image collection around the world used in  more than 65\% research publications in the past 20 years \cite{BILJECKI2021104217}. A majority of the images provide 360-degrees panoramic (with a few exception when narrow roads are surveys by foot using backpack-mounted cameras). The service is currently active in more than 90 countries with recent expansion to some indoor spaces. The GSV API provides access to images to its users in pay-as-you go model. The easy access, omnidirectionality and coverage are the major factors for Google SVI's popularity.

\subsection{Crowdsourced Street View Datasets} \label{sec:background_crowd}
Other notable services providing access to street view images collect images through crowdsourcing. Two such services, Mapillary and KartaView, provide commercial access to their images covering several locations around the world. 

\paragraph{KartaView}Founded in 2009 and originally called OpenStreetView (later OpenStreetCam) it is currently owned by Grab Holdings. Users can capture video from the Android or iOS App or upload images separately. Images are licensed CC BY-SA 4.0, meaning users can share and adapt as long as they give attribution and use a similar license. As of May 24, 2021, KartaView claimed it had 384 million images ``covering almost 8 million kilometers of road'' \cite{craciun_2021}.
\paragraph{Mapillary}
Founded in 2013 and purchased by Facebook (now Meta) in 2020, Mapillary data is also licensed CC BY-SA. As of December 2021, Mapillary claimed it had 1.5 billion images and ``more than 10 million kilometers'' \cite{quack_2021}. Mapillary also produces an SDK, a web interface for analysis, and pre-computes object detections for hundreds of traffic signs and 42 other standard objects in their images.

\smallskip
 Due to the reliance on public contributors for images, these services have some significant differences from images available via GSV. Unlike GSV where locations are typically revisited approximately once a year, crowdsourced images can be of much higher temporal resolution, especially for areas frequented by many people. % frequently at different times. 

There are several limitations of these data. First, crowdsourced images are taken by different users, rather than collected from standardized  LIDAR-equipped dedicated GSV cars. Hence the images are not panoramic 360 images; in most cases, the datasets only feature a front view of the road. Various devices are used to collect the images, resulting in datasets with heterogeneous quality. Spatial coverage of the data is variable, as the locations captured tend to be opportunistic rather than strategic. % receive fewer visits and interests from pedestrians, cyclists and motorists. 
This may result in a mapping of the city that is less comprehensive than that of GSV but updated more often.

%For this research, we focus on high frequency street view data



% Seeing urban environments is challenging due to the wide variety of scale and context necessary. Local governments might need regular data on a large geographic area while community groups may need higher fidelity data on only a few blocks. A real estate developer may need specific measurements of a singular block. Street View Imagery is increasingly used\cite{biljecki2021street} along with sensor networks\cite{rashid2016applications}, satellite imagery \cite{miller2003cities}, urban ethnography \cite{jackson1985urban} and survey/census data \cite{logan2018relying}. 

% I wonder if a table here makes sense? for the different modalities? 


 
%  In our current research, PIs Ortiz, Ju, and Pierson have successfully used vehicle-data from Nexar Ltd. to recognize people and estimate pedestrian traffic and physical distancing behavior in COVID-19 New York \cite{ju2020tracking}.

% \subsubsection{Satellite Images} Satellite imagery, combined with geographical information systems have been used to perform city-scale analysis and present the results as a map. This allows producing macro level insights by automatically extracting micro level information from the pixels of the image. Google Earth and Sentinel Hub are two common data sources providing commercial access to their data products. There are several other government owned data-sources such as USGS EarthExplorer, National Oceanic and Atmospheric Administration (NOAA), and NASA Worldview, etc. While each of these services provide free access for non-commercial applications, limited access to open data products only, poor resolution, low update frequency and pricing are the key challenges for using satellite imagery in studying urban life.

% \subsubsection{Street View Images} While aerial images can provide useful information about overall urban infrastructure through a perspective from above, seeing the city landscape from a ground level perspective analogous to human vision provide more fine-grained information. From images captured at street level, urban developers can use these micro level information from an urban scene, classify them into different components of built environment, and statistically evaluate different parts of the city for policy making purpose. As mentioned above, 

% Unlike, other notable services providing access to street view images collect images through crowdsourcing. Two such services, Mapillary and KartaView provide commercial access to their images covering several locations around the world. Due to the reliance on public as contributor for images, these services have some significant differences from images available via GSV. Unlike GSV where locations are revisited once approximately once a year, crowdsourced images can be of much higher temporal resolution specially for areas visited by a lot of people frequently at different times. However, there are several limitations for these data. First, as crowdsourced images are taken by different users, unlike the standardized collection method with lidar equipped dedicated GSV cars, the images are not panaromic, rather front view of the road in most cases. This also leads to highly heterogeneous quality of the images due to various device types used in collecting the images. Spatial coverage of the data is another concern in this case as some locations that receives fewer visits and interests from pedestrians, cyclists and motorists. This results into a mapping of the city that is less comprehensive that that of GSV.

% There are also several other local instances of street view image services such as Tencent (China), Microsoft Bing Maps, Cyclomedia (Europe), Yandex (Russia), etc. which provide access to street view images accessible to specific corresponding country. 

 \subsection{Hardware Manufacturer Street View Projects} \label{sec:backgorund_oem}

Automotive Original Equipment Manufacturers (OEMs) and add-on manufacturers have collected street view imagery via networked dash cameras reporting to a central service. They are similar to crowdsourced images in that they can be collected at a much higher temporal resolution than services collected by single companies, such as GSV, but with less variability than is typical in crowdsourced street view projects. 

\paragraph{Nexar}
Nexar manufactures internet connected dash-cams often used by drivers for insurance claims. Using data collected from dash cams, Nexar is producing a digital twin for real-time road data. Images are processed and objects are detected for work zones, traffic, and road signs. As of July 2022, Nexar's website claims the company has collected over 1.5 billion miles of data, producing 4 terabytes of images which users can interact with on their CityStream platform.
\paragraph{MobilEye}
Founded in 1999 and acquired by Intel in 2017, MobilEye is primarily focused on autonomous driving and advanced driver-assistance systems (ADAS). MobilEye manufactures hardware used in vehicles from six OEMs, with over 1 million vehicles collecting street view data covering 25 million kilometers per day \cite{korosec_2022}. The data is not visual but extracted text snippets representing road objects and conditions. MobilEye sell data services for road asset mapping, change detection, and dynamic mobility datasets.


\begin{figure}[t]
     \centering
          \begin{subfigure}[b]{0.3\textwidth}
         \centering
         \includegraphics[width=\textwidth]{Figures/mapillary_example.png}
         \caption{Mapillary}
         \label{fig:mapillary_ex}
     \end{subfigure}
     \hfill
     \begin{subfigure}[b]{0.3\textwidth}
         \centering
         \includegraphics[width=\textwidth]{Figures/nexar_example.jpg}
         \caption{Nexar}
         \label{fig:nexar_ex}
     \end{subfigure}
     \hfill
     \begin{subfigure}[b]{0.3\textwidth}
         \centering
         \includegraphics[width=\textwidth, trim={0 0 0 6.5cm},clip]{Figures/kartaview.png}
         \caption{KartaView}
         \label{fig:karta_ex}
     \end{subfigure}
     \caption{Example images from various street view datasets}
\end{figure}

\section{Applications of Street View Image Datasets}

Street view images open opportunities for urban researchers and policy makers to use the images as a virtual representation of the street scenes in the real-world.   Street View Imagery is increasingly used \cite{biljecki2021street} along with sensor networks \cite{rashid2016applications}, satellite imagery \cite{miller2003cities}, urban ethnography \cite{jackson1985urban} and survey/census data \cite{logan2018relying}. These datasets suit a wide variety of uses: Local governments might need regular data on a large geographic area while community groups may need higher fidelity data on only a few blocks. A real estate developer may need specific measurements of a singular block.   %which is useful for gaining insights about street events from a specific point scale to even city scale. 
Urban planning and social science studies have used street view images as a proxy for traditional survey methods, so that researchers can analyze activity without directly observing the streets to collect data \cite{shapiro2018street, vandeviver2014applying}.%However, this work is distributed across numerous academic and professional communities, and this work is intended to pull these interdisciplinary perspectives together. 

\subsection{Street View Images in Urban Computing} \label{sec:background_urban_computing}

Collecting data at a city scale is a time-consuming and expensive, yet an essential step for urban analysis. Street view images have been useful for gaining urban-scale insights. Nuanced information extracted from image content is a unique data resource.

GSV images have been used to classify urban street features such as trees \cite{thirlwell2020big, 8930566}, utility poles \cite{krylov2018automatic}, traffic signs \cite{campbell2019detecting, 10.1145/3180496.3180638}, bike racks \cite{maddalena2020mapping} and manholes \cite{vishnani2020manhole} in an effort to map their distribution across the city. Similarly, the images have been used to estimate road quality and classify road surface types \cite{zhang2020automatic, doi:10.1177/2399808319828734}, sidewalk mapping \cite{doi:10.1177/2399808321995817} along with detecting and classifying potholes and other defects \cite{9072401}. Classifying land use and urban zones based on their operation (residential, industrial, etc.) is another avenue of work along this line \cite{feng2018urban, chang2020mapping}. To categorize different parts of a city based on commercial activity, researchers have leveraged commercial establishments and points of interest from street images \cite{10.1145/3184558.3186581, 8890683}. Street view images have been used to predict building age \cite{li2018estimating}, heights, use and architectural style \cite{hoffmann2019model, GONZALEZ2020106805}. Images have been useful in urban energy forecasting \cite{guhathakurta2020spatial}. 
% Relationship of road aesthetics (road objects, greenery) to citizen travel behavior have been explored in \cite{YANG2020102442, 10.1145/3289600.3290611}.

% Transportation and mobility studies are another application area where street view images have been frequently used. 
As pedestrian and cycling safety has been a major concern in urban design, attributes such as number of lanes \cite{cicchino2020not}, sidewalk width and surface have been studied using street view images to explore their relationship to crashes and falls \cite{isola2019google}. Street view images have been found useful for computing car driving difficulty \cite{skurowski2018saliency} and pedestrian volume \cite{chen2020estimating}. Mobility patterns and route choices for cyclists and pedestrians may be captured with street view images \cite{wang2020relationship, goel2018estimating, verhoeven2018differences} .
 Street view imagery have been used in efforts to study the relationship the built environment and  the spread of infectious diseases such as dengue fever \cite{andersson2019combining} and COVID-19 Flu \cite{ijerph17176359}. Street view images have shown promises in estimating sun glare, sky view, light pollution, shade percentage, etc. \cite{gong2018mapping, liang2020gsv2svf, zeng2018fast}. 

In recent years, street view images have been used to quantify greenery, walkability, and physical attractiveness to study their links to various health outcomes such as happiness \cite{hart2018contextual}, obesity and physical activity \cite{hart2018contextual}, air quality \cite{doi:10.1021/acs.est.0c05572}, and mental health \cite{wang2019urban}. Massive spatial coverage in these datasets has been useful in studying urban walkability and accessibility based on crowdedness~\cite{cao2018walkway,weld2019deep, zhang2018walking}. GSV images have been used in accessing property value by extracting neighbourhood and available amenities \cite{law2019take, bin2020multi, fu2019street}. As physical attributes of a neighborhood can be a reliable indicator of socio-economic factors, street view images were used in studies to predict income \cite{diou2018image} and crime rates \cite{Vandeviver2014ApplyingGM}.

\subsection{Human centered urban studies with street view images} \label{sec:background_human_centered}

The advent of big data in urban planning and design benefit urban studies in a human centered manner through exploring interventions and their impacts at both city and individual scale. 

% However, such exploration require tools that allow practitioners to interact and visualize large data sets collected across cities to understand urban fabric and reimagine its future.

Urban studies have traditionally relied on field visits and audits to tackle questions concerning the built environment's impact on public health, pedestrian fatalities, perception of safety, etc \cite{RePEc:sae:urbstu:v:45:y:2008:i:9:p:1973-1996, sallis2012role, CLIFTON200795}. Creative, interactive tools to support the works of professionals for improving the design and experience of urban built environments has garnered attention among the HCI and CSCW coummunities. Earlier works by White et al. \cite{10.1145/1518701.1518871} and Underkoffler et al. \cite{10.1145/302979.303114} introduced systems to integrate field visit data with existing maps on a unified platform for ease of comprehension and analysis. With the emergence of large scale image data set such as GSV Images as a new data source that is capable of offering dense representation of geographic locations both spatially and temporally, researchers have started to utilize these images in urban design work, particularly for auditing and validating the built environments. Progress in computer vision has enabled processing and querying large scale image data sets for virtual audits \cite{10.1145/2647868.2654948, https://doi.org/10.48550/arxiv.1404.1777, lowe2004distinctive}. This has the potential to scale up auditing process for urban planning with wider coverage, as a substitute for time-consuming and labor-intensive physical site visits. 

Increasingly, there are efforts to incorporate public input in urban design processes and engage communities in design interventions \cite{10.1145/3173574.3173769, 10.1145/3290605.3300571}. Large scale virtual auditing requires expert input in labeling and street users often lack that kind expertise. To mitigate this gap, \cite{10.1145/3290605.3300292} used crowdsourcing to label accessibility issues on GSV images. However, creating tools and methods to visually explore such urban scale data poses new challenges. To aid visual analysis of spatio-temporal data on air pollution, mobility, and transportation, a number of visual analytical tools have been proposed \cite{4376168, 10.1145/3183713.3193559, 7390069, 6876029, 6634127, 7539380, 10.1145/2557500.2557537}. 

% In a parallel line, using computer vision based automated information processing, several methods introduced have used satellite and street view images to predict the relationship of theurban built environment attributes such as greenery, sky view, land use, visual aesthetics, etc. with health outcomes, socio-economic conditions, street safety, etc.  
% However, as GSV images are temporally sparse typically, its usefulness is limited when practitioners want to study the temporal evolution of a specific location. Recently, street view images captured by dashboard cameras mounted on regular vehicles making trips on the street have become a new data source to address this gap. There are several companies such as Carmera, Nexar, and Hivemapper which collect such information on several major cities. The use of this kind of \emph{in-the-wild} dataset to explore built environment's influence on quality of urban life has been limited, with an exception of \cite{miranda2020urban}, where  Miranda et al. studied visual aspects of street to understand issues such accessibility and mobility. The work done in this paper focus on this particular type of dataset, which we believe has the potential to be informative to studying many nuanced layers of urban living and aid in urban design in a data-driven manner at a lower cost.

\subsection{Social sensing using street view images}

% While there are many modalities to sense the world at a large scale, images has been found to be information-rich  are attractive for analytics purpose because of this reason. While there are other sensing modalities that have been used successfully for smart city application in the built environment such as sound, RF frequency, etc., we limit our discussion in this paper to specifically for images, particularly the ones used for studying urban life. To understand the built environment, there are two types of data that are available for urban planners and policy makers: Remote sensing such as satellite imagery, and On street sensing through street view imagery. 

Machine learning and computer vision, along with high-performance computing, allow storage and processing of large collection of images, which can be useful for analyzing changes captured over a long period, or for comparing similar contexts in different cities or continents. The deployment of computer vision recognition at scale that makes it possible to use street view images for "social sensing"--analysis of how people's use of cities ebbs and flows over time \cite{liu2015social}.  %Scene understanding can also discern the qualitative composition of physical spaces throughout the city, traffic, and under varied climatic conditions[reference?].

Prior research has used datasets from fixed public web cameras to track individuals and groups in urban spaces and estimate their movement patterns \cite{slobogin2002public, hipp2016webcams, seer2014kinects} and pedestrian volume \cite{liu2009pedestrian, petrasova2019visualization}. Researchers at Voxel51, for instance, are using computer vision analysis on public web-camera data to track the impact of COVID on social behavior using a metric they call the Voxel51 Physical Distancing Index (PDI)~\cite{casalmoore_2020}. These cameras run at a frame-rate that allows every person in their view to be counted; however, these cameras are sparsely distributed throughout urban spaces.

Vehicle-mounted cameras can observe people over a larger area. Zhang et al used 120k street-level images of the streets within the Ring Road of Beijing to estimate the spatio-temporal distribution of taxi trips \cite{zhang2019social}. Kataoka et al. used cameras on vehicles driving through urban and suburban areas to characterize the walking activity well enough to predict pedestrian intent \cite{kataoka2015fine}.  Research on pedestrian detection from vehicles has been greatly aided by datasets of dense pedestrian activity captured from dash-camera footage under various conditions, such as~\cite{DBLP:journals/corr/abs-1909-12118}. 

\subsection{Privacy and data governance for street view images} \label{sec:background_privacy}

While street view image can be a valuable services for many urban applications, legitimate privacy concerns exist about its capability of revealing sensitive information. The images are taken from public spaces and images available over platforms such GSV can be accessed by anyone in the world with internet access. Furthermore, the possibility of these image collections being used as a proxy for representing events and observations of real world (e.g. mobility, health and well-being, etc.) for critical policy-making calls for attention to ensure the portrayal of the society and trustworthiness in the data.

In an early effort to individual privacy in street view image, Google introduced an automatic blurring method to mask face and license places present in their images \cite{35481}. Street view images, like any other digital photography available to public over the internet, can reveal sensitive information even from fractional information available of  pedestrians and vehicles; hence, further methods were proposed from a computer vision standpoint to automatically remove such objects as if they never existed in the scene \cite{https://doi.org/10.48550/arxiv.1903.11532, 5543255, nodari2012digita}. While Google has introduced reporting mechanism to remove photo containing sensitive and inappropriate content, legal and privacy scholars have found the wide coverage and universal access to the data to be of concerns as it can be used for malicious attempts such as stalking, facilitating crimes, and compromising privacy \cite{Rakower}. Lack of online image management, which is an individual's ability to define their image and its use on the internet with adequate consent, threatens a person's integrity, reputation, and the essential right to privacy. 

% Contextual integrity suggests that privacy depends is based on appropriate information flow which depends on context \cite{10.5555/1822585}, meaning some information may be considered as private in one context while being considered as public information in another. However, 
Under ecosystems of Surveillance Capitalism \cite{zuboff2019age}, companies like Google with its access to user data on a personal level through its array of products along with its services mapping cities, can infer insights and modify behaviors without asking permission. The question of data governance, which is the process to manage availability, usability, integrity, and security of the data, becomes a challenge when big data are used in decision making systems \cite{JANSSEN2020101493}, such as when GSV images are used as virtual proxy for human observations \cite{curtis2013using}. Street view imagery that are not accessible to public also pose the risk of being misused if made available through paid license to third-party services. 

% Previous work has established that ostensibly public information poses meaningful risks to personal privacy, including public records \cite{martin2017privacy}. Even in its anonymized form, this data presents a re-identification risk. Previous work by de Montjoye et al. indicates that in an anonymized, granular dataset of location traces, it is possible to re-identify 95\% of individuals using only two spatio-temporal points where a specific person was known to be \cite{de2013unique}. Furthermore, the image-based nature of this data and the recent proliferation of readily-available facial recognition technology deepens the privacy risks of the data used in this project. \cite{brey2004ethical,best2007facial} In this strand of the work, we describe how this work will contribute to research on responsible data use by applying a contextual integrity theory of privacy to data sharing practice \cite{nissenbaum2009privacy}.

There are several harms made possible by the collection and storage of identifiable data, contingent on whether the data is subject to a security breach or misused. Widespread street-level data collection may violate public expectations of privacy through obscurity, that is, the sense that information is relatively safe as long as it is hard to obtain or understand  \cite{hartzog2015surveillance}). The combination of widespread data collection, storage, and analytic tools reduce the cost of eliciting details previously protected by obscurity \cite{zimmer2008externalities}. Street-level information about individuals' behavior can reveal sensitive details, such as who someone is, what they are doing, and who accompanied them at a particular place and time \cite{rakower2011blurred}. 

% \subsection{}

% \section{Background}

% \subsection{growth in data size}
% \subsection{companies and organizations}
% \subsection{comparison to GSV}
% \subsection{comparison to satellite imagery}


==> v1_CSCW/03_methods.tex <==
\section{Expert Perspectives on Street View Image Datasets}
To determine some of the challenges and opportunities presented by large scale street view datasets, we performed a series of interviews with experts in urban planning, analytics, and design from the New York City area. We focus on novel higher temporal frequency datasets such as those described in sections  \ref{sec:background_crowd} and \ref{sec:backgorund_oem}. We grounded the discussion with a demonstration of a specific New York dataset; experts were chosen from the New York area because they would have familiarity with the territory covered by the exemplar dataset. %r. 
Participants were chosen for their expertise in studying urban environments at various scales, from single sites to neighborhoods to entire cities.

We performed interviews with: 
\begin{itemize}
    % DFTA
    \item \textit{P1:} A senior executive and a research scientist from the NYC Department for the Aging (DFTA).
     % Nneka
    \item \textit{P2:} An Urban Designer and Civic tech entrepreneur with experience of building tools for the NYC Department of City Planning.
    % Kurt
    \item \textit{P3:} An Urban Planner from and VP of planning for the Flatiron Nomad Partnership Business Improvement District (BID).
   % Tom
    \item \textit{P4:} An assistant professor of Civil and Mechanical Engineering focused on using mobile sensing technologies to monitor urban and structural environments.
    % Wenwen
    \item \textit{P5:} An assistant professor of informatics with a focus on urban simulation, land use and transportation interaction.

\end{itemize}
Each interview lasted approximately an hour and was conducted by two authors simultaneously over Zoom. Interviews covered the expert's background, past usage of street view datasets, and views on potential usage of data within their own professional work. To ground the discussion, we showed participants images from a large scale data-set of dashcam data collected by Nexar, shown in Figure \ref{fig:nexar_ex}. %Participants were asked about their current exposure to and use of street view imagery. Participants were shown examples of dashcam footage and asked to discuss potential uses within their current workflows. 

% TODO nexar images

Interviews were semi-structured and took place in 2021 and 2022. All interviews took place and were recorded over Zoom. Two authors on the paper were present at each interview. Two authors independently labeled transcripts of the interviews for emergent themes, using a grounded theory approach. Emergent codes and themes were developed individually, and then iteratively discussed, refined, and grouped in an open coding process \cite{khandkar2009open, braun2006using}. %Themes were discussed and merged as necessary until a consensus was reached.

==> v1_CSCW/04_findings.tex <==
\section{Findings}
We identify a number of themes  related to the differences between participant approaches to novel datasets, previous experience with street view imagery, and the application areas they explore around the potential uses of dash cam street view imagery. Participants regularly framed the challenges and opportunities relative to their experience with existing datasets such as GSV. While several of the challenges noted are not unique to street view imagery, these challenges are often exacerbated by the data-set sizes and the quality variance presented by dash-cam footage. We present the findings below.

\subsection{Financial Cost} \label{sec:findings_cost}
Deciding to use a data product is intimately related to its cost. Cost of access and cost of use can be prohibitive to organizations, particularly when researchers are uncertain if they will be able to extract relevant outputs.

% \subsubsection{ Costs}

P2 described the selection and procurement process at the New York Department of City Planning:
\textit{\begin{quote}
    There were a few times where [we used] proprietary data sets. However, they were either just too expensive for a city budget and you have to go through a whole procurement process that can open up a can of worms... Trying to assess, how much value we would really get for this proprietary data? Is it really worth that cost? Whether it's a financial cost or the labor costs of doing this procurement process.
\end{quote}}

Government resources are limited and data procurement involved enough work that it was often better to ``scale back [P2's] expectations or scope of our work and still kind of generally get to the right direction, of the kind of analysis we're trying to do with just open data sets.'' Data for governmental, non-profit, or community organizations would better serve the public if the data is permissively licensed or easily accessible to researchers and urban planners who might work in these areas.

The issue of cost was echoed in P5's description of changes in GSV data from free data to a limited and priced credit system:
\textit{\begin{quote}
    Google started to charge for images. That made a huge difference for academics who want to use it...  Now I think  [GSV] account only gives users  200 credits per month.
\end{quote}}

The restrictions on data usage affected the degree to which academics could rely on GSV and motivated a turn to other sources. When operating with access to large resources in a collaboration on a well-funded project, P5 described the affiliates that enable bulk downloads of GSV data:
\textit{\begin{quote}
    [They] were rich enough to say `I want all the data'...  it's a company that works closely with Google, for people to get a large quantity of the data. The first million images is expensive, but additional millions of images is much cheaper. [This] gives researchers less motivation to query the data.
\end{quote}}

The pricing structure described above is designed to encourage bulk downloading. The result is to privilege institutions with pre-existing relationships with large corporations, large onsite or cloud storage facilities, access to a supercomputer, and a predetermined question rather than exploratory analysis.

P4 noted how costing processes change as a dataset becomes more useful:
\textit{\begin{quote}
     The value of a data set changes based on the competition. There's also a barrier, where, if [the data] gets too expensive, people are just going to not care anymore, and find another way to do it. Or start collecting data [themselves]. ... If it's free and low-hanging fruit, it's really exciting because there seems like there is big potential. Once that paywall gets introduced ... it seems to be less useful. It seems to just fall into the business bottle of some company and then it's a black hole.
\end{quote}}

Proprietary datasets are already being used in the service of generating a profit while permissively licensed datasets are currently owned by large corporations with no guarantees those datasets will remain openly accessible. 

% \subsubsection{Computational Costs}
% \subsubsection{Labor Costs}
% Choices on data sources and types to use are 
% \subsection{Expertise and Infrastructure}  \label{sec:findings_infrastructure}

\subsection{Static vs Dynamic Spatial Attributes}  \label{sec:dynamic}

Participants focused on application areas that were suited to lower quality images with much higher update frequencies. These were often brought up in direct contrast to GSV. Google cars typically revisit a street around once or twice a year, often optimizing for times when the street is the least busy. This limits the ability to use their data for understanding aspects of the urban environment that change faster than that or focusing on people and objects moving through the space rather than aspects that are fixed and infrastructural.

P3 described sending staff weekly to survey charges to retail spaces on the ground level, currently taking up to 20 person-hours of labor a week using ``a spreadsheet they actually print out and walk around with and check on things''. While P3 had recently used street view to check ``if there were manhole covers on the street'' which were covered in snow at the time, P3 stated that their staff would ``never lean on it for on-the-ground measurements or anything.'' GSV is a tool primarily for when they are ``being lazy'' or viewing something far from the district. However, P3 and their organization find value in real-time data sources when insights were extracted for them. 


Using a service called Spring-Board, three cameras installed at high angles in parks are used for pedestrian counts \cite{springboard_2022}. Given the use of existing statically mounted cameras, there is a clear use case for pedestrian tracking and understanding foot traffic behavior in this Business Improvement District.

The eye-level perspective of SVI allows for a better understanding and analysis of fine-grained human behavior in space than street view datasets captured from high angles. P2 described: % how part of the job of an urban designer included:
\textit{\begin{quote}
   [Part of the job of an urban designer is understanding] how do people move through the space. Do you notice that a lot of people sit there? Are there always constantly groups of people sitting around? Or is there always a steady flow of people walking through the space? I would also [pay attention to] cyclists. Are there any cyclists moving through space? Are they locking their bikes anywhere?
\end{quote}}

As discussed in Section \ref{sec:background}, fine-grained canvasing is historically labor-intensive, and demands an observer to be on-site  for extended periods of time. Higher frequency capture of street view imagery may open up new methods for urban analysis at scale.

P3 described several observations that would have been easier to deduce via street view imagery rather than manual counts.
\textit{\begin{quote}
    While [looking at] quantity counts of bike traffic in the district during the summer, I expected that people would be biking in the morning and evening. In reality, it was actually lunchtime and evening. What I realized pretty quickly was the bike traffic was largely commercial cyclists at lunchtime, making deliveries. We also saw that Broadway was about 25\% bidirectional biking even though it's a one-way facility. People are using it both ways because it's so convenient as a diagonal.
\end{quote}}

Urban environments are used in ways that were not originally intended. Better instrumentation of the urban landscape allows the urban design to adapt to the norms people develop as they move about space. P3 continued to describe how they hoped to add additional bike parking in response to the massive influx of food delivery workers. Being able to capture and query this kind of data on demand would aid that process.

Participants described other counter-intuitive temporal data that they believed could be extracted from street view imagery. Describing the need for increased granularity to assist older adults, P1 mentioned this:
\textit{\begin{quote}
     [Beyond bi-weekly updates], it could be even more granular. Even time of the day. If [an elderly person] live[s] across the street from a school, most of the time walking in that community is not a problem. But when the kids are leaving school at three o'clock or right before school starts there's no way that [they] can get access. It could even be more granular a whole day, it could be times of the day... [also] seasonality. This block could be fine nine months out of the year, but three months out of the year, it's treacherous.
\end{quote}}
 
 Temporal granularity can raise causal relationships that might otherwise be challenging to deduce. Seeing exemplar data that is updated in near real-time led P1 to suggest building new kinds of tooling that could assist elderly inhabitants to decide when to leave or how to navigate the city that takes their unique needs into account.
 
 Higher update imagery can also benefit urban populations more generally. P5 noted how urban developments such as ride-sharing and e-scooters have complicated how cities prioritize curb use:
\textit{ \begin{quote}
     [Another field] developing very rapidly is curbside parking, or curb use. It has become a very popular problem, especially after the introduction of micro-mobilities [scooters and e-bikes], and Uber. You frequently see Uber drivers double-park, loading and unloading. A lot of places are trying to get rid of on-street parking which frees up the curb spaces [reserved for] loading and unloading only. It's a very vague criteria. How do you define how long people park there? What would be considered as loading and unloading? Is sitting there for 30 minutes loading or unloading? That's very hard to decide...[these kinds of] reinforcement things would benefit from images that update more frequently
 \end{quote}}
 
%  So all those kind of reinforcement thing would benefit from the image that is updating and also like the real-time traffic information that will be extracted and all the congestion, emission data that can be. provided on those kind of image will be also very valuable... there are projects that try to predict air quality based on Google Street View image. Then if it's updated every second, every minute, it will have better air quality model.

Of the many use cases for street view imagery discussed in section \ref{sec:background}, many of them would benefit from higher frequency data if the underlying signal extracted changes at a time frame greater than the once every 6-12 months GSV and related projects typically re-image a street. P5 added that ``projects that try to predict air quality based on Google Street View images, if it's updated every minute, will result in a better air quality model.''

Similar to the examples mentioned in section \ref{sec:background_urban_computing}, changes in street assets due to damage were raised by P4, P3, and P5. P3 and P5 mentioned that many municipalities have no consistent database of traffic signs. If one is knocked over in the Flatiron District,  P3 or someone from their team reaches out to the Department of Transportation to get it fixed. 

Some of these opportunities can and are being done today such as using street view imagery to better keep track of road and traffic signs\cite{nexar_2022} or curb usage \cite{nexar_2022}.

\subsection{Interacting with images at scale} \label{sec:findings_image_scale}
Large amounts of image data provide unique challenges to both the quantitative and qualitative analytical methodologies used by our participants. This includes data exploration, storage, labeling, filtering, querying and reporting. 

P2 further describes the importance of street view imagery and the failure in tooling to bring together imagery and analysis that urban planners can use:
\textit{\begin{quote}
    The reason why a lot of photos are required for city planning or zoning applications is because you can read a lot from photos of places in the city. I just haven't seen yet a lot of tools that make that connection. [Tools that try] to further analyze the data that [urban planners] are reading from these photos. 
\end{quote}}

% I think oftentimes a lot of its inferred or it just has to be written out exactly what's what's valuable about this particular image.

Until tooling improves the opportunities for urban analysis at scale is unlikely to occur. Urban planners and analysts need methods for approaching large datasets that can be queried and clustered for use patterns. 

P2 described how making tools for community organizations required simple clear outputs that could be used with little modification:
\textit{\begin{quote}
    [Community board members] weren't data experts per se, they just have these reports. The biggest challenge that they had is that the open data portal seemed overwhelming. They're not comfortable with spreadsheets. They have these reports, but they're often outdated. The reports [may not contain] the specific types of data that they want to report. Instead of saying the top three languages spoken, they want to be able to at least have the option to provide top 15 languages spoken in their neighborhood, and that may not have been provided. That particular audience honestly just want the visualization...to maybe copy and paste specific data points that were helpful for their work. They were also able to easily create screenshots of graphs, or custom maps...that they can put in their report. That was really valuable for them.
\end{quote}}

For users less confident in interacting with large datasets `` the biggest value was really the ability to visualize data and do some slight customization of like maps and graphs'' (P2).

The process P2 described aligned with the approach taken by P3 which involved a number of tools that take complex inputs and produce direct readable reports stating ``we're still pretty dependent on the dashboards that we actually pay for and we keep those reports''. P2 mentioned Spring-board which uses mounted cameras and computer vision to generate pedestrian counts. CoStar merges a variety of public information to generate reports on real estate. Placer.ai is used to estimate foot traffic in the neighborhood. StreetPlus generates a data dashboard for waste management. These services are paid for and used to simplify data collection and analysis by a team that is small and unlikely to employ a data scientist.
 
P1 considered the utility of being able to query images which could then be used for ``validating that data with older adults and workshops where [we would like to ask participants ]`Hey can you point out some problematic areas for us?' ''. The opportunity presented allows street view imagery to be leveraged as a probe to better discuss the challenges of elderly residents, challenges which may or may not be reflected in the existing data.
% Our experts came from a range of backgrounds with various amounts of exposure to data science. 

Visual data often requires labeling to extract information not captured by simple heuristics. This is a well-explored challenge in HCI, CSCW, and AI communities which some of our participants have first-hand experience with. For simple labeling tasks, P5 is having Mechanical Turk workers draw bounding boxes around e-scooters. For more complex tasks, P5 describes:
\textit{\begin{quote}
    We have been using Mechanical Turk to label the sample data to develop machine learning models using Street View to predict Local Climate Zone... Mechanical Turk is highly scalable. We can gather those results fairly quickly, but the quality of the results is not comparable with expert labeling.
\end{quote}}

A significant amount of work is necessary to make street view datasets usable. For features without obvious heuristics, each labeling task will differ based on the application. If each feature of interest requires expert labeling, the likelihood of widespread use is limited. 

% \subsection{Ethical Concerns}  \label{sec:findings_ethics}

% The datasets being described are urban surveillance at a massive scale. Ethical concerns brought up existed primarily along two tracks. There were concerns about maintaining privacy and the potential reduced utility of the datasets that might pose. The other theme that was brought up was data equity and curation. Given that these datasets are collected from vehicles the limit is areas where there may be fewer cars. In particular Nexar has many dash-cams mounted in ride-share vehicles which many not serve all areas.

\subsection{Privacy} \label{sec:findings_privacy}

In general, participants approached the datasets as an opportunity in their own work and were less concerned with some of the significant privacy violations made possible by such massive imagery datasets.

P2 was a key exception to that pattern. While P2 had described much of the value of street view imagery as being related to how the imagery captures people interacting in public, P2 were also hesitant. P2 described how standard privacy mitigation for public imagery may be insufficient:
\textit{\begin{quote}
    Even though faces might be blurred, because this data is captured at a higher frequency, it's still easy to see patterns. For people living on [a] block, you might see them ... multiple times a day.  I do think that blurring faces isn't enough in addressing privacy. It requires the obscuring of people in general. Because again, you're able to start picking up on patterns and triangulating data.
\end{quote}}

 Given P2's background working with the government and with community groups, underrepresented minorities and people of color, they were the most concerned about the potential for privacy abuses by state, corporate and individual actors. Maintaining privacy is an important area that will require additional study if large scale street view datasets are to be made a viable resource for urban studies.

Longstanding concerns around privacy with GSV were discussed in section \ref{sec:background_privacy}. Many of these concerns may be exacerbated as the size of these datasets grow; the temptation to use these large-scale urban datasets "for good" with the belief that such uses can be separated from the bad uses still seems to prevail. 

P5, for example, seemed critical of privacy protections, and seemed to indicate that more surveillance could be used to address crime. 
\textit{\begin{quote}
    [Be]cause United States doesn't have a security surveillance system due to privacy protections, sometimes you really need, those kind of images to, know whether a crime really happened. Or if a crime happened, where that person went. If you have good coverage and videos that is updated frequently enough, you can leverage it as a security system for the city.
\end{quote}}

 To us, this is an indicator that researchers and planners who have access to large scale urban datasets might, with only good intentions, enable data usage that violates people's civil liberties if potential abuses are insufficiently managed. This type of misuse should be anticipated and addressed %The desire to use these tools for the enforcement of a carceral state will need to be taken into account 
 by those that produce, release, and sell these datasets.

\subsection{Data Equity and Curation}
% \subsubsection{Access and Resource Equity}
If data is being used to make claims, and enact policy changes, it requires guarantees about its completeness and distribution. Data needs to be collected such that it controls for temporal and spatial differences. If an area is being sampled more frequently end users should be able to easily control for that in their analysis to reduce oversampling bias. 

P4 referred to previous work that showed:
\textit{\begin{quote}
    If [researchers randomly put a sensor on 30 taxis, within 24 hours it would cover every block [in Manhattan] so just pick 30 taxis at random and that's all it would take to at least get to each block once, roughly speaking of course.
\end{quote}}

Increasing the number of sensors placed on vehicles increases both the spatial and temporal frequency of data collection. This is one approach to ensuring data is widely cross-applicable.

When working on a project, P2 described the process of curating interviews: 
\textit{\begin{quote}
    [Curating interviews require being] strategic and finding specific people who, represent broadly across different demographics. When I talked to city planners...  I tried to find people of different demographics, people of color, older people, younger people... Not only do we identify the most appropriate people for our work but we're trying to make sure we have a broad cross-section of demographics when inviting people for interviews.
\end{quote}}

P2 is suggesting that the same approach to curating interviews in more ethnographically focused work could provide an approach to the curating of street view datasets. Collect images that target the specific groups, locations, and demographics necessary to effectively answer the question rather than attempting to collect any and all data available with the expectation that it will immediately be useful.
% Curating interview subjects as a model for intentionality in dataset curation is reflected in some of P2's concerns with how data around walkability is typically defined rather than used in practice.
\textit{\begin{quote}
     [Often] the way that walkability is calculated isn't actually a helpful way to assess particular subgroups of walkers like elderly people.  I find that that circumstance is true for lots of other city residents ...I've personally experienced how limited data can be because, it's either captured in a way that's just too broad, or that it is only really relevant for an athletic young male  city dweller.
\end{quote}}

When large datasets are utilized to determine whether a metric that might be ageist, ablest or presupposes a norm, it doesn't matter how large the data originally was. P2 points out:
\
\textit{\begin{quote}
    [It is better to] not just have more data available, but to specifically toggle to specific subsets of demographics. [Finding] data that's most relevant to those subsets would be really helpful. Trying to understand what demographic subsets can you then find specific data around? and what are the limitations of that kind of data? ... Being able to capture and find data that's most relevant to very specific groups of people is helpful.
\end{quote}}

% , and can now then open up a whole floodgate of very like different ways and metrics that are most relevant to that data group that could just be like really difficult to be able to capture in a very accurate or consistent basis 

P2 suggests targeted street view data collection rather than aggregate collection. Specifying regions to intentionally address specific research or planning questions would reduce some of the costs (storage, compute, labor) and challenges of working with these datasets while allowing researchers to make equity claims directly when curating a dataset.

==> v1_CSCW/05_discussion.tex <==
\section{Discussion}

\subsection{Cost and Availability} \label{sec:discussion_cost}
The period of free access to GSV demonstrated applications and use cases that GSV's current cost structure no longer supports. There are therefore opportunities for parties who can provide open-source or low-cost datasets to fulfill urban planning, analysis, and research needs.  P5 mentioned how the change in Google street view pricing affected their research.
As several participants mentioned, high costs for evaluating the quality and potential value of street view data present barriers to the use of SVI by urban planning professionals.   

The list of existing high-frequency street view data providers includes permissively licensed images collected by crowd-workers, and proprietary data collected by sensors installed by OEMs and aftermarket vehicle products. The growth of public datasets could parallel the arc of freely available high-frequency remote observation data from sources such as Landsat, and the Copernicus Program. These datasets have resulted in numerous publications in urban studies and planning \cite{cetin2019effect, deliry2021extracting, fu2019characterizing, jutz2020copernicus, tapete2018appraisal, kuc2019sentinel} as well as other fields. The value of this data likely led to much of the growth of the private and commercial remote observation industry \cite{dehqanzada2000secrets, wulder2019current}. 
% ranging from agriculture \cite{}, OSINT \cite{}, finance and international relations

\subsection{Tooling and Interfaces}
% continue in the challenges discussed when it comes to tools and interfaces for high frequency street view imagery. Both are massive image datasets that can be difficult to work with.
Interacting with large imagery datasets of all kinds remains challenging. While there have been some approaches as discussed in section \ref{sec:background_human_centered}, images can be noisy, and require large amounts of storage and processing power for analysis. While deep learning techniques for image analysis, segmentation, and object recognition have improved significantly since the 2010's \cite{alom2018history}, many challenges remain when problem areas aren't tightly bounded, which is often the case in urban analysis.
Some of the parallels to satellite imagery observations in section \ref{sec:discussion_cost} are also productive for developing the space of tools and interfaces for street view datasets. Similar to the field of remote observation, the data is imagery in massive quantities. The mode of analysis is often exploratory and may require expert labeling. Both satellite and street view imagery raise persistent privacy concerns that individuals, states, and corporations will be forced to navigate. Some of the tooling that has been developed by the remote observation community points towards similar approaches that might scale to the challenges of street view imagery.

Platforms and infrastructure such as Google Earth Engine \cite{gorelick2017google} and Sentinel Hub \cite{milcinski2017sentinel} demonstrate how massive parallel computing can be made easy and accessible to novices democratizing analysis. They also include pricing structures that make non-commercial, academic and government use affordable or free further incentivizing their use.

More accessible and collaborative software for generating custom maps \cite{kastanakis2016mapbox, felt, placemark} is beginning  to address some of the requirements of community organizations as described by P2 and P3. Some data providers are beginning to integrate tooling for custom maps, filtering by object detection, and easier data exploration. While these tools are still limited, %object detections are only available from predetermined categories. S
some of the exact problems and uses described by P3 and P5, such as curbside detection, are already beginning to be offered by companies such as Nexar \cite{nexar_2021}. We can expect these tools to continue to improve and add functionality.
\begin{figure}[t]
     \centering
     \begin{subfigure}[b]{0.48\textwidth}
         \centering
         \includegraphics[width=\textwidth]{Figures/mapillary_filters.png}
         \caption{Mapillary filtering for cars, bicycles, and cyclists \cite{mapillary_2019}}
         \label{fig:mapillary_od}
     \end{subfigure}
     \hfill
     \begin{subfigure}[b]{0.46\textwidth}
         \centering
         \includegraphics[width=\textwidth]{Figures/nexar_filters.png}
         \caption{Nexar CityStream filtering for traffic signs \cite{nexar_2022}}
         \label{fig:nexar_citystream}
     \end{subfigure}
     \caption{Filtering for detected objects}
\end{figure}

\subsection{Value and Quality of Street View Imagery} 

Images contain `general-purpose' information with many use cases. However, the quality of crowd-sourced images varies due to heterogeneity in device, orientation, and occlusions. Data collected in uncontrolled settings can show spatial, temporal, and content distribution variance. Images may be of sufficient quality for some applications while needing a higher quality score for others. Collecting more information or maximizing coverage does not guarantee improved data quality. For example, air quality changes slowly, so a higher sampling frequency may not add more value to the data in regular environmental sensing applications. Evaluating the value and relevancy of data is essential to justify the monetary and labor investment urban professionals need to sanction before incorporating such large-scale datasets into their analysis workflow.

Quality of Information in a sensor network is a metric used to evaluate information to make decisions about the utility of a specific piece of information \cite{10.1145/2489253.2489265}. It is the difference between observed measurements of an event via sensing and the actual measurement \cite{4660116, 10.1016/j.cageo.2021.104991}.
Frameworks have been proposed for scoring and ranking generic information based on spatio-temporal context, accessibility, trustworthiness, data provenance, timeliness, presentation, and relevance as key characteristics to evaluate application-specific utility \cite{10.1145/2489253.2489265}. Existing approaches have developed application-specific frameworks by ranking sensors according to task relevancy and user requirements  \cite{8606228, 6935003, 7295461, 7348644}. 
The quality of coverage thus depends on the velocity, mobility pattern, and the number of sensors available \cite{10.1145/1161089.1161102}. Existing work has explored adaptive spatial sampling for optimizing value and cost \cite{BALLARI2012102, NGAI2014203}, and detecting missing points in data to improve coverage \cite{wang2006movement}. Most existing works focus on spatial coverage, and little work on Quality of Information has focused on temporal coverage, where events of interest need to be observed multiple times within a time interval.  
The large volume of data generated by such vehicular networks is a challenge due to the processing and storage requirements. These may be mitigated by querying and filtering data points below certain information quality (e.g. filtering images in dark, occlusion, blurriness, etc. conditions). Data-driven mechanisms need to be formulated to localize data segments with low information quality and incentive mechanisms produced to improve the quality of captured imagery~\cite{10.1145/2888398}.

\begin{figure}
  \includegraphics[width=0.5\linewidth]{Figures/blurry_image.jpg}
  \caption{An example of a Nexar image, whose blurriness would lead to low QOI for many applications.}
  \label{fig:nexar_low_QoI}
\end{figure}


% hile some services such as GSV ensure spatial coverage updated approximately least once per year, data collected at this frequency can  be less relevant to detect changes in urban aspects that change at a faster temporal rate. On the other hand, w

% When multiple instances of the same event are captured, the Quality of Information for each capture must be determined to decide which instance is prioritized. This is particularly challenging when sensor samples are images, whose content may be of high quality and relevancy for one context while providing low information value for another (e.g. image of the same road intersection showing the potholes of the street may be less valuable for pedestrian counting applications). 

% It is closely related to Value of Information \cite{article12}, a concept to assess the utility of information for a specific purpose.
% , and Age of Information \cite{yates2021age} which is the concept of timeliness of information delivery. 
% Quality of information can be regarded as context-independent whereas the value of information is context-dependent. Even high information quality can offer low information value for a specific application \cite{4144841, bisdikian2007quality} 
% (e.g. temperature data at minute resolution for transit design).  
% As the definition of information value is dependent on the specific purpose where it is used, evaluating the Quality of Information across multiple applications is challenging. 


% Quality of Information is influenced by external environmental factors, 


% The quality of information from mobile sensing systems that capture, street view images is dependent on the dynamism inherent in the network.


% As spatiotemporal data collected by vehicular networks, street view image data can be considered a form of participatory sensing \cite{burke2006participatory, 10.1145/2888398}. As humans and external factors such as social, economic, and cultural context are major actors in the data collection, trustworthiness, reliability, and consistency needed for adequate information quality is crucial as outlined in \cite{10.1145/3139256}. 


% Although there are various Quality of Information measures proposed in the literature that can be useful for sensing data at a city scale, there is little work to measure information quality for Spatio-temporal data. It is particularly challenging when the data is collected in image form as information quality that can be extracted from an image is application specific. It is becoming increasingly popular to use computer vision to automatically extract information from large-scale street datasets to develop insights for planning and policies. Without a proper mechanism to evaluate the quality and value of the data for the task in hand, the data can provide an incomplete understanding of the city and its population leading to unfair policies and planning decisions.



\subsection{Privacy and Equity}
Privacy concerns with on-street image collection have a long precedent as discussed in section \ref{sec:background_privacy}. Most publicly licensed street view imagery (Mapillary and KartaView) have followed Google's precedent, blurring faces and identifiable information. While P2 considered the removal of all people from images to mitigate privacy concerns as discussed in section \ref{sec:findings_privacy}, many of their suggested use cases would conflict with that. For example, SVI datasets can have such high spatial density and image frequency that a person could be tracked via their clothing even if their face is blurred. Further work is necessary to understand the potential privacy harms that high frequency street view data might pose. Existing approaches to mitigate privacy harms--such as similar pedestrian substitution \cite{nodari2012digital} or image-to-image translation \cite{xiong2019privacy}--may also be applicable to these datasets. Furthermore, we should acknowledge there are sensitive sites-- parenthood clinics, dispensaries, bars, playgrounds-- that present risk to different populations around which active regulation of data collection may be necessary.

One of the benefits of imagery at this scale and temporal frequency is the ability to capture data on demand when you need it for a specific research goal rather than storing everything. On the other hand, for things like understanding historical trends or response to specific events--like how people respond to a public health curfew in different neighborhoods--having caches of data going back to specific times can be very useful. In some ways, having collections of "normal" behavior, lightly sampled, and adding temporal resolution and density of coverage when patterns are unusual is what might be most useful for detecting urban patterns and responding proactively to new issues or patterns. 

Ensuring fresh and equitable imagery will require broad infrastructural investment or  a well-formulated incentive structure for crowd-contributed data. Mapillary has a marketplace and ``Missions'' to fund and gamify data capture \cite{quack_2021}. Both KartaView and Mapillary publicly display leaderboards to encourage participation and data collection. These incentive structures may help but are insufficient with Mapillary still showing significant inequality in data captured \cite{ma2019state}. Collaborations with fleets and state agencies that already have consistent and full coverage may help guarantee more equitable coverage \cite{yoong_2018}.

% Notes from chat
% this is stuff that you can just collect on demand (privacy). GSV is secondary use, it can be useful or abusive. If you can get a lot of data on demand you can capture the data on demand when you need it. On the other hand, for things like understanding historical trends or response for specific events--like how people respond to a public health curfew in different neighborhoods--having caches of data going back to specific times can be very useful. In some ways, having collections of "normal" behavior, lightly sampled, and adding temporal resolution and density of coverage when patterns are unusual is what might be most useful for detecting urban patterns and responding proactively to new issues or patterns. 

%Otherwise, having filters on for commonly abusable information which enables individual level tracking and having some log of people who ask to pull requests for that data to be off might be helpful for having people think twice about hoarding potentially abusable information, and at least encouraging accountability and transparency about how the data is used.


% I think it’s worth saying that it is possible to have loss of privacy, but that the likelihood of catching any specific person using these methods is low, since the capture of individuals with these methods is serendipitous.
% Nevertheless there are sensitive sites—parenthood clinics, dispensaries, bars, playgrounds—that we should be mindful might present risk to different populations, and hence some proactive anticipation and mediation of possible issues is necessary




==> v1_CSCW/06_conclusion.tex <==
\section{Conclusion}
Intersecting trends including excitement over autonomous vehicles, ride-sharing growth, OEMs integrating cameras into vehicles, and the increasing availability of cheap and ubiquitous connected devices have resulted in significant growth in the availability of street view imagery. These images vary in licensing, quality, and update frequency. We present an overview of the challenges and opportunities these novel datasets might present to urban planners and researchers, to help research and product based on SVI to serve better the needs of people who are working on city services and planning. We have reviewed current offerings of street view imagery and brought together relevant research that applies the analysis of street view imagery to problems in urban planning. To better inform the development of services and research with the needs of urban planners and researchers, we performed interviews with an array of experts working in this domain. 

Experts we interviewed clearly saw new kinds of questions this data could help them explore, and valuable services this data could help them provide to urban residents. Additionally, they expressed concerns about developing and using high frequency street view datasets. These include the challenges of integrating new datasets into existing workflows, data equity, and privacy. For quantitative researchers, the cost of large scale data in acquisition and processing was raised. For qualitative researchers, interfaces for understanding and easily querying street view images are likely necessary. We believe these user-centered insights on the challenges and opportunities of street view imagery for urban planning and analysis will help researchers in the CSCW community to build tools to support community-centered work. %These datasets present opportunities for the HCI and CSCW communities to explore designing for and with these datasets for urban communities taking the work from labs and data providers in a more user centered direction.

% Advances in image processing techniques for tasks such as object detection, segmentation, and scene classification, along with dramatically cheaper digital storage, has increased the accessibility and utility of these large street view datasets. While researchers and companies providers are ramping up what is possible using these services, few of those researchers seem to be directly in touch with the prospective users of these tools and services in the domain of urban planning. Hence, this work seeks to aid the advancement of this promising area in a more use-inspired direction.

